Hierarchical Diffusion Autoencoders and Disentangled Image Manipulation

Diffusion models have attained impressive visual quality for image synthesis. However, how to interpret and manipulate the latent space of diffusion models has not been extensively explored. Prior work diffusion autoencoders encode the semantic representations into a semantic latent code, which fails to reflect the rich information of details and the intrinsic feature hierarchy. To mitigate those limitations, we propose Hierarchical Diffusion Autoencoders (HDAE) that exploit the fine-grained-to-abstract and lowlevel-to-high-level feature hierarchy for the latent space of diffusion models. The hierarchical latent space of HDAE inherently encodes different abstract levels of semantics and provides more comprehensive semantic representations. In addition, we propose a truncated-feature-based approach for disentangled image manipulation. We demonstrate the effectiveness of our proposed approach with extensive experiments and applications on image reconstruction, style mixing, controllable interpolation, detail-preserving and disentangled image manipulation, and multi-modal semantic image synthesis.

==> figs_rebuttal/fig_empirical_plot.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.75\linewidth]{figs_rebuttal/empirical_plot.png}
    \vskip -0.1in
    \caption{
        % \textbf{Ablation study of different architecture designs.}
        % We plot the curves for MSE and LPIPS metrics on the validation set during training.
        %HDAE(E) only uses one third of the baseline DAE training time to outperform DAE on the inversion quality. And HDAE(U) outperforms HDAE(E) and the original baseline DAE on the inversion quality at the same training steps (1,020K steps). 
    }
    \vskip -0.12in
    \label{fig_empirical_plot}
\end{figure}

==> figs_rebuttal/ir_ug.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=1\linewidth]{figs_rebuttal/ir_ug.pdf}
    \vskip -0.1in
    \caption{
        More results will be added in the final version.
        % \textbf{Ablation study of different architecture designs.}
        % We plot the curves for MSE and LPIPS metrics on the validation set during training.
        %HDAE(E) only uses one third of the baseline DAE training time to outperform DAE on the inversion quality. And HDAE(U) outperforms HDAE(E) and the original baseline DAE on the inversion quality at the same training steps (1,020K steps). 
    }
    \vskip -0.15in
    \label{ir_ug}
\end{figure}

==> figs_rebuttal/topk.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.8\linewidth]{figs_rebuttal/topk.pdf}
    \vskip -0.15in
    \caption{
        % \textbf{Ablation study of different architecture designs.}
        % We plot the curves for MSE and LPIPS metrics on the validation set during training.
        %HDAE(E) only uses one third of the baseline DAE training time to outperform DAE on the inversion quality. And HDAE(U) outperforms HDAE(E) and the original baseline DAE on the inversion quality at the same training steps (1,020K steps). 
    }
    \vskip -0.2in
    \label{topk}
\end{figure}

==> figs_rebuttal/user_study.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.8\linewidth]{figs_rebuttal/user_study.pdf}
    \vskip -0.15in
    \caption{
        % \textbf{Ablation study of different architecture designs.}
        % We plot the curves for MSE and LPIPS metrics on the validation set during training.
        %HDAE(E) only uses one third of the baseline DAE training time to outperform DAE on the inversion quality. And HDAE(U) outperforms HDAE(E) and the original baseline DAE on the inversion quality at the same training steps (1,020K steps). 
    }
    \vskip -0.15in
    \label{user_study}
\end{figure}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> section/00_abstract_original.tex <==
\begin{abstract}
\vspace{-1pt}
% Abstract goes here.
%\xihui{TODO.}
%In view of the dazzling performance of denoising diffusion probabilistic models (DDPMs) in the field of image generation, DDPMs have been extensively studied in various computer vision tasks.
Diffusion models have attained impressive visual quality for image synthesis.
However, how to probe and manipulate the latent space of diffusion models has not been extensively explored.
Prior work diffusion autoencoders encode the semantic representations with a single latent code, neglecting the low-level details and leading to entangled representations.
To mitigate those limitations, we propose Hierarchical Diffusion Autoencoders (HDAE) that exploits the coarse-to-fine feature hierarchy for the latent space of diffusion models.
Our HDAE converges 2+ times faster and encodes richer and more comprehensive coarse-to-fine representations of images.
The hierarchical latent space inherently disentangles different semantic levels of features.
Furthermore, we propose a truncated feature based approach for disentangled image manipulation.
We demonstrate the effectiveness of our proposed HDAE with extensive experiments and applications on image reconstruction, style mixing, controllable interpolation, image editing, and multi-modal semantic image synthesis.
The code will be released upon acceptance.
%Diffusion Autoencoders (DAE) can separately infer both semantics and stochastic information from an input image.
%Our motivation is to connect the seminal idea of multiscale features with DAE.
%In this work, we present Multiscale Diffusion Autoencoders which involve the multiscale semantic vectors to complement the latent space with multiscale information. 
%Firstly, we explore five kinds of latent spaces with singlescale or multiscale semantic features, dubbed E space, E+ space, ED space, ED+ space and ED++ space respectively. 
% E+ space only uses one third of the baseline E space training time to outperform E space on the image reconstruction quality. %%%% Need modify
%E+ space only uses one third of the training time the baseline E space dose, but outperforms E space on the image reconstruction quality.
%%%%
%And ED+ space outperforms both E+ space and the original baseline E space at the same training steps (120M steps).
%Then we propose a novel editing method where users can manually adjust the degree of disentanglement.
%Extensive experiments and applications show a clear improvement in training efficiency, reconstruction quality and editing quality.
\end{abstract}

==> section/01_intro_original.tex <==
\vspace{-12pt}
\section{Introduction}

%% wordings:
%% pave the way to 
%% disentanglement is inherent
%% it is critical to explicitly decouple the information of different layers
% ommiting the rich information in the low-level and mid-level features
% feature vectors extracted from various spatial levels of the encoder can correspond to different semantic levels of details of the diffusion-based decoder, achieving semantic correspondence and reducing training difficulty
% different semantic/abstraction levels of features
% encode/capture rich hierarchical semantics
% 


Diffusion models~\cite{DDPM,DULNT} have demonstrated impressive image generation quality and
%They are able to produce a wide variety of highly realistic synthetic images.
%There are various studies to further improve DDPMs in both theory a00nd practice \cite{ImproveNCSN,AnalyticDPM,ADM,EDM,IDDPM}.
%In addition, DDPMs are also used in other computer vision tasks, such as text-to-image generation\cite{DALLE2,GLIDE}, image editing \cite{p2p, DAE, Dreambooth, MCF, diffusionclip}, image inpainting \cite{repaint,NTIRE}. 
achieved remarkable success in various applications, such as text-to-image generation~\cite{DALLE2,GLIDE}, image editing~\cite{p2p, DAE, Dreambooth}, and inpainting~\cite{repaint,NTIRE}.

A semantically meaningful, editable, and decodable latent space is of particular importance in interpreting generative models as well as applications such as image editing.
There have been various works on designing and manipulating the latent space of GANs~\cite{Interfacegan,SeFa,GANspace}.
However, the latent space of diffusion models has been underexplored.
Preechakul~\etal proposed Diffusion Autoencoders (DAE)~\cite{DAE}, which leverages a learnable encoder to discover high-level semantic representations and leverages a diffusion model to encode the stochastic variations and decode images from the semantic latent code and the stochastic latent code.
%Recently, Preechakul proposed Diffusion Autoencoders\cite{DAE}, termed as \textbf{DAE}, to utilize a learnable encoder for discovering high-level semantic representation vector $z_{s}$ and utilize DDIM\cite{DDIM} for decoding and modeling stochastic variations $x_T$.
%Concretely, we first obtain high-level semantic representation vectors $z_{s}$ from feature maps encoded by semantic encoder.
%%%% Need modify
%Then we condition the diffusion unet using adaptive group normalization layer (AdaGN)\cite{ADM} on the high-level semantic representation vectors $z_{s}$.
%%%%
%After getting the high-level semantic representation vector $z_{s}$, we can modify the semantic representation vector $z_{s}$ according to the direction from a trained attribute classifier.
%Using the modified or original high-level semantics representation vector $z_{s}$ and stochastic variations $x_T$, we can generate a highly realistic synthetic image.

However, the semantic latent code of diffusion autoencoders is simply represented by a single feature vector predicted by the last layer features of the semantic encoder, ignoring the rich low-level and mid-level features. Such a latent space is insufficient to encode the rich information from images.
%The na\"ive latent space is not only insufficient to encode all of the coarse-to-fine visual representations of an image, but also entangled with different attributes. 
%As a result, the image reconstruction is inaccurate and  different attributes cannot be disentangled from the simple latent space.
In practice, we observe that the fine-grained representations (\eg, background and low-level details) are omitted by the semantic encoder and only encoded by the stochastic encoder, leading to difficulties in manipulating those fine attributes.
%Furthermore, the holistic latent code leads to entanglement of different attributes (\eg, ``old'' is entangled with ``wearing eyeglasses''), and it is difficult to find a single direction to manipulate a specific attribute without affecting other attributes.
Furthermore, different levels of representations are entangled within the single holistic semantic latent code, making it difficult to find a single direction in the latent space to manipulate a specific attribute without affecting other attributes.

%However, due to the latent space design of the Diffusion Autoencoders, the learned semantic representation vector $z_{s}$ is insufficient to express the information contained in the input data. 
%If we simply use $z_{s}$ encoded by semantic encoder and a random $x_T$ sampled from gaussion distribution to reconstruct the original image, there is a large gap between the reconstructed image and the original image, as shown in Fig. \ref{Reconstruct} and Tab. \ref{imgrectab}.
%At the same time, $z_{s}$ is often entangled in some directions for the simple latent space.

%Meanwhile, the computer vision community developed multiscale processing involved in some key papers by Rosenfeld and Thurston~\cite{ECDVSA}, Burt and Adelson~\cite{TLPCIC}.
%The motivation of multiscale processing is to take advantage of contextual semantic information at different scales.
%Feature maps at different scales contain different semantic information.
%The high-resolution feature maps contain low-level semantic information and the low-resolution feature maps contain high-level semantic information.

To mitigate those problems, we design the \textbf{Hierarchical Diffusion Autoencoders (HDAE)} that exploits the coarse-to-fine feature hierarchy of the semantic encoder and the diffusion-based decoder for comprehensive and disentangled representations.
Our design of the hierarchical latent space is motivated by the observation that feature maps at different scales correspond to different abstraction levels of features.
The high-resolution feature maps contain low-level features (\eg, color, texture, and details) and the low-resolution feature maps contain high-level features (\eg, structure, layout, abstract attributes).
In particular, we extract different levels of features from the semantic encoder and use them to predict the semantic latent code for the corresponding feature levels of the diffusion-based decoder.
We extensively investigate different design choices of HDAE, as demonstrated in Fig.\ref{overview}.
%, and find the optimal U-Net structure leading to accelerated training and rich semantic representations.
Our HDAE converges three times faster than DAE~\cite{DAE}.
Image reconstruction and image editing experiments demonstrate that the latent representations of HDAE are richer and more comprehensive than DAE.
Moreover, the different semantic levels of features are inherently disentangled in the hierarchical latent space, and we probe the hierarchical latent space with style mixing and controllable image interpolation experiments.
%Diffusion models apply a u-net structure at each time step, where an encoder encodes the noisy image into a low-resolution feature map, and then a decoder decodes a less noisy image from the feature map.
%Motivated by this observation, we extract different levels of features from the image encoder, and feed them to the diffusion model.
%With deliberate design and experiments on different structures of the hierarchical diffusion autoencoders, we find the optimal structure leading to accelerated training and more comprehensive feature representations.
%With the latent space with rich hierarchical semantics, we achieve better image reconstruction and image editing quality than diffusion autoencoders and GAN inversion approaches.
%The latent space hierarchy is illustrated through style mixing and controllable interpolation experiments.


%In this work, our motivation is to connect the seminal idea of multiscale features with Diffusion Autoencoders~\cite{DAE}. 
% We start from semantic representation to explore five kinds of latent spaces, dubbed E space, E+ space, ED space, ED+ space and ED++ space respectively. 
% Concretely, we firstly obtain high-level semantic representation vectors $z_{s}$ from feature maps encoded by semantic encoder.
% Then we condition the diffusion unet using adaptive group normalization layer (AdaGN)\cite{ADM} on the high-level semantic representation vectors $z_{s}$.
%Based on the idea of multiscale, we design three multiscale latent spaces: E+ space, ED+ space and ED++ space.
%In addition, we compare two singlescale latent spaces: E space and ED space.
%We evaluate these five latent spaces on FFHQ dataset~\cite{Stylegan} using image reconstruction %quality, as shown in Fig. \ref{ablationplot}.
%Finally, we obtain the following conclusions:
%%%% Need modify
%(1) Multiscale Diffusion Autoencoders is an efficient learner: E+ space only uses one third of the baseline E space training time to outperform E space.
%%%%
% unet like architecture semantic encoder
%(2) unet~\cite{unet} like architecture semantic encoder cannot directly improve the performance of Diffusion Autoencoders: E space and ED space are almost the same on LPIPS~\cite{LPIPS} and MSE.
%(3) unet like architecture semantic encoder can improve performance with Multiscale Diffusion Autoencoders: ED+ space outperforms both E+ space and the original baseline E space at the same training steps (120M steps).

%A critical issue for image manipulation with generative models is the entanglement of different attributes.
To further improve the disentanglement of attributes for image manipulation,
%We find the hierarchical latent space naturally provides disentangled features: global and abstract attributes are controlled by the high-level features, while local and detailed attributes are controlled by the low-level features.
we propose to conduct manipulation with truncated features, based on the observation that the majority, low-value feature channels are a critical cause of entanglement.
Experiments demonstrate that the truncated features facilitate disentangled attribute manipulation of face images, \eg, we can disentangle ``old'' from ``wearing eyeglasses'' so as to edit a face image towards older without adding eyeglasses to the face.

%\xihui{Disentanglement of features.}

%Generally speaking, there are two major advantages to use multiscale semantic features.
%Firstly, we evaluate Multiscale Diffusion Autoencoders from the perspectives of both inversion quality and image editing. 
%DAE(ED+) achieves state-of-the-art performance, as shown in Tab. \ref{imgrectab} and Fig. \ref{facemanipulate}.
%Secondly, semantic vectors of different scales encode different semantic information, as shown in Fig. \ref{interpolation}.
%Based on the multiscale semantic features, we propose a novel editing method where users can manually adjust the degree of disentanglement.

%\xihui{summary}

% the generative representations learned by the GANs with layer-wise latent codes are specialized to synthesize different hierarchical semantics
% By probing the layer-wise representations with a broad set of semantics at different abstraction levels, we are able to quantify the causality between the activations and semantics occurring in the output image


In summary, we propose Hierarchical Diffusion Autoencoders which exploits the coarse-to-fine features to obtain a comprehensive and disentangled latent space for diffusion models. We further propose a novel approach for disentangled attribute manipulation with truncated features.
Experiments are conducted on FFHQ, CelebA-HQ, and LSUN Cat datasets. 
We demonstrate that our model can capture rich and disentangled semantic representations with extensive experiments on image reconstruction, style mixing, controllable image interpolation, disentangled image editing, and multi-modal semantic image synthesis, as shown in Fig.\ref{teaser}.
%The effectiveness of the hierarchical latent space is demonstrated with image reconstruction, style mixing, and latent space interpolation experiments. We also illustrate that our approach can disentangle attributes for image editing.

\label{sec:intro}


==> section/04_method_.tex <==
%\section{Method}


\subsection{Hierarchical Diffusion Autoencoders}\label{subsec:hierarchical}

\input{figs/clsheatmap}

%Although Diffusion Autoencoders~\cite{DAE} can produce very accurate reconstruction results with the semantic vector $z_{s}$ and the stochastic vector $x_T$, its reconstruction results are weak without the stochastic vector $x_T$, as shown in Fig. \ref{Reconstruct}.
%In image synthesis models, the visual features at different levels follow a coarse-to-fine hierarchy.
The semantic latent code in diffusion autoencoders is a single 512-dimensional feature vector, encoding different semantic levels of features from coarse and abstract features to fine-grained, low-level features.
Such semantic representations bring two limitations. 
Firstly, the single feature vector from the final layer of the semantic encoder omits the low-level and mid-level features. And it is not sufficient to encode the comprehensive semantic information in the images.
Secondly, different levels of representations are encoded in the single feature vector, making it difficult to disentangle different attributes for image editing.
%Empirically, we observe that the images reconstruction and editing results with diffusion autoencoders suffer from insufficient details and inconsistent identities.
%It demonstrates that the information contained in the semantic vector $z_{s}$ is insufficient to represent the image $x_0$.
%And the identity of the reconstructed image is not similar to the identity of the original image.
%We attribute this problem to the latent space design of the Diffusion Autoencoders.

To address those issues, we propose hierarchical diffusion autoencoders which explore the hierarchical semantic latent space of diffusion autoencoders.
In particular, we explore the design space of diffusion autoencoders and hierarchical diffusion autoencoders, as shown in Fig.~\ref{overview}.

\noindent\textbf{Diffusion autoencoders, denoted as DAE.}
The diffusion autoencoders~\cite{DAE} leverage a semantic encoder with downsampling layers.
%, and leverages the feature.
%However, the last layer output of the encoder is not sufficient for encoding all semantic representations, from low-level to abstract level.

\noindent\textbf{Diffusion autoencoders with U-Net semantic encoder, denoted as DAE(U).}
We replace the downsampling encoder in DAE with a U-Net encoder, denoted by DAE(U).
With the skip connections and downsampling-upsampling design, the last layer of the U-Net might be able to capture both low-level and high-level features.
The spatial feature map from the last layer of the U-Net is mapped into a 512-dimensional feature vector $z_s$ with a global average pooling layer followed by a fully-connected layer.
However, experiments indicate that DAE(U) does not perform better than DAE.
%We further design three architectures with hierarchical latent space: HDAE, HDAE(U) and HDAE(U+).

%We construct five kinds of latent spaces for Diffusion Autoencoders (DAE)~\cite{DAE}, dubbed DAE, DAE(U), HDAE, HDAE(U) and HDAE(U+) respectively, as shown in Fig.\ref{overview}.

%We first introduce two non-hierarchical latent spaces: DAE and DAE(U).
%DAE is the latent space used by original Diffusion Autoencoders.
%As shown in Fig. \ref{overview}, it uses a semantic encoder with feature map resolution decreasing layer by layer to extract visual feature.
%Then the feature map from semantic encoder is fed into \textbf{map module} which learns to map the $2D$ spatial feature to a $1D$ vector $z_{s}$ of dimension $d=512$.
%Unlike DAE, DAE(U) uses the u-net~\cite{unet} like architecture semantic encoder.
%Here we use the same architecture as \textbf{diffusion u-net} from ADM~\cite{ADM}, but remove the last resblock, dubbed \textbf{semantic u-net}.
%Then the feature map from the last resblock is fed into the map module to get the semantic vector $z_{s}$.
%After getting the $z_{s}$, the vector is used to modulate the output feature maps of each convolutional layer in diffusion u-net with AdaGN~\cite{ADM}.
%begin{align}
%    AdaGN(h, y, z_{sem}) = z_{s} ( y_{s} GroupNorm(h) + y_{b} )
%\end{align}
%where $h$ is the intermediate activations of the residual block following the first convolution and $y = [y_s, y_b]$ is obtained from a linear projection of the timestep.

%Then we introduce three hierarchical latent spaces:  HDAE, HDAE(U) and HDAE(U+).
\noindent\textbf{Hierarchical diffusion autoencoders with simple semantic encoder, denoted as HDAE(E).}
To exploit the feature hierarchy of the diffusion autoencoders,
we extract different semantic levels of feature maps from the semantic encoder to predict the hierarchical semantic latent codes $z_s^1, z_s^2, \cdots, z_s^L$.
The different levels of semantic features are fed into the corresponding levels of the diffusion-based decoder.
%The semantic features from the high-resolution layers of the semantic encoder contain low-level features, and are used as the conditions of the high-resolution layers of the diffusion model.
%Likewise, the semantic features extracted from the low-resolution layers of the semantic encoder encodes abstract visual representations, and are fed into the diffusion model as the conditions of the low-resolution layers.

%We divide diffusion u-net and semantic u-net into $2L$ blocks according to the size of the feature map ($L$ is the feature map number of different size in diffusion u-net).
%Diffusion u-net takes latent codes $c = \left \{ c_e^{l}, c_d^{l} \right \}^L_{l=1} $ as the input of AdaGN.
%$c_e^l$ represents latent code required by the $l$th block in the encoder of diffusion u-net and %$c_d^l$ represents latent code required by the $l$th block in the decoder of diffusion u-net.

%As shown in Fig. \ref{overview}, HDAE space uses the same semantic encoder as the original Diffusion Autoencoders.
%But HDAE does not only obtain one semantic vector of dimension $d=512$ from the last resblock in the encoder through the map module.
%For feature map $F^l$ from the $l$th block divided by the size of the feature map, we feed $F^l$ into a map module to get one semantic vector $z^l$  of dimension $d=512$.
%So we can get the semantic vectors $z_s = \left \{ z^{l}\right \}^L_{l=1}$.
%For the latent codes required by the diffusion u-net, we have $ c_e^{l} = c_d^{L-l+1} = z^{l} $.

\noindent\textbf{Hierarchical diffusion autoencoders with U-Net semantic encoder, denoted as HDAE(U).}
HDAE(U) shares the same hierarchical latent space design as HDAE but leverages a semantic encoder with the U-Net structure.
%For feature map $F_d^l$ from the $l$th block in the decoder of the semantic u-net, we feed $F_{d}^{l}$ into a map module to get one semantic vector $z_{d}^{l}$ of dimension $d=512$.
%So we can get the semantic vectors $z_s = \left \{ z_{d}^{l} \right \}^L_{l=1} $.
%For the latent codes required by the diffusion u-net, we have $ c_e^{L-l+1} = c_d^{l} = z_{d}^{l} $.

\noindent\textbf{Hierarchical diffusion autoencoders with U-Net encoder plus, denoted as HDAE(U+).}
%HDAE(U+) uses the same encoder (semantic u-net) as the DAE(U) and HDAE(U).
%For feature map $F_{e}^{l}$ and $F_{d}^{l}$ from the $l$th block in the encoder and decoder of the semantic u-net, we feed $F_{e}^{l}$ and $F_{d}^{l}$ into map module to get semantic vectors $z_{e}^{l}$ and $z_{d}^{l}$.
%So we can get the semantic vectors $z_s = \left \{ z_e^{l}, z_{d}^{l} \right \}^L_{l=1} $.
%For the latent codes required by the diffusion u-net, we have $ c_e^{l} = z_{e}^{l}$ and $c_d^{l} = z_{d}^{l} $.
We further propose HDAE(U+), where the U-Net semantic encoder predicts $2L$ semantic latent codes to feed into the corresponding layers of the diffusion-based decoder, as shown in Fig.~\ref{overview}.


Experiments demonstrate that the hierarchical structures HDAE(E), HDAE(U), and HDAE(U+) provide richer semantic representations and more efficient training than DAE and DAE(U). 
The hierarchical representations are also more controllable for image editing because they contain comprehensive coarse-to-fine features. In contrast, the representations of DAE only contain high-level features, and the low-level features of DAE are encoded in the stochastic latent code $x_T$ which is difficult to control.
%In DAE, the stochastic details are encoded in $x_T$, which we cannot control. In our three versions of HDAE, however, most details are also encoded in the semantic vectors, leading to more controllable image editing.



%There are two major advantages to use hierarchical semantic features.
%Firstly, the image synthesized by diffusion u-net can be completely determined by hierarchical semantic vectors $z_{s}$ without any other variations, making them suitable to express the information contained in the input data without stochastic vector $x_T$. 
%Secondly, as shown in Fig. \ref{interpolation}, semantic vectors of different scales encode different semantic information.
%The semantic vectors corresponding to coarse spatial resolutions($8^2\sim16^2$) encode high-level semantic information such as pose, gender, face shape, and eyeglasses.
%The semantic vectors corresponding to high spatial resolutions($32^2\sim256^2$) encode low-level semantic information such as color scheme, smaller scale facial features and microstructure.

\subsection{Disentanged Latent Representations}\label{subsec:space}
% Shen et at. proposed InterFaceGAN to achieve real image manipulation.
% Suppose we have a semantic scoring function $f_S: \mathcal{X} \rightarrow \mathcal{S} $, where $S\in \mathbb{R}^m$ represents the semantic space with $m$ semantics. 
% We can bridge the latent space $\mathcal{Z}$ and the semantic space $\mathcal{S}$ with $s = f_S(g(z))$, where s and z denote the semantic scores and the sampled latent code respectively.


%Shen~\etal~\cite{Interfacegan} proposed InterFaceGAN to achieve real image manipulation:
With a linear classifier trained with the semantic vectors, diffusion autoencoders~\cite{DAE} can be applied for image editing.
We can edit an image by moving the semantic vector towards the direction $n$, which is obtained from the weights of the linear classifier for the target attribute.
%With diffusion autoencoders, we can find such a direction $n$ from the weight vector of a linear classifier trained on latent codes of negative and positive images of a target attribute, e.g., old.
%To manipulate the attribute of a synthesized image, we can easily edit the original latent code $z$ with $z_{edit} = z+\alpha n$.
%This operation can continuously change the semantic attribute in the image.


\input{figs/directionbarmap}

%We first train the Hierarchical Diffusion Autoencoders on FFHQ~\cite{Stylegan} of image size 128 × 128. 
%After that, we fix the Hierarchical Diffusion Autoencoders and train the classifier on CelebA-HQ~\cite{ProGAN} of image size 128 × 128.
In our HDAE models, the dimensions of the semantic latent vectors are $512\times 5$. We flatten the semantic vectors to a single vector of dimension $2560$, and derive the classifier direction $n\in\mathbb{R}^{2560}$.
We calculate the normalized classifier weights $\hat{n}$ as follows:
%So the dimensions of the latent code $z$ and normalized classifier direction $n$ are $2560$ (Here $L = 5$, $512 \times 5 =2560$ ).
%And we can get normalized classifier direction $\hat{n}$ as follows:
\begin{align}
    \hat{n}_i = \frac{|n_i| - \underset{i}{\operatorname{min}}(|n_i|)} {\underset{i}{\operatorname{max}}(|n_i|) - \underset{i}{\operatorname{min}}(|n_i|)}
\end{align}

\input{figs/topkmanipulate}

We visualize the values of the $5\times512$-dimensional normalized classifier weights $\hat{n}$ in Fig.~\ref{clsheatmap}.
We observe a clear pattern that most high values of a specific attribute are concentrated in one or two levels, indicating a strong correlation between feature levels and attributes. For instance, the color attribute ``brown hair'' is correlated with the low-level feature layers 1 and 2, while the abstract attribute ``smiling'' is correlated with the high-level feature layer 4.
This phenomenon indicates that the hierarchical latent space can capture coarse-to-fine features, and different layers represent different levels of semantic representations.
%As shown in Fig.\ref{clsheatmap}, we visualized the normalized classifier direction $\hat{n}$ according to the layer.
%The normalized classifier directions of most layers are relatively low, but $1 \sim 2$ layers are notable.
%On the one hand, it shows that some attributes are associated with some layers.
%%%% Need modify
%For example, as shown in Fig.\ref{clsheatmap}, "Hair Cheekbones" and "Smiling" are associated with the second layer, "Brown Hair" with the fifth layer, and "Eyeglasses" with the first layer.
%%%%
%On the other hand, it shows that different layers can express different semantic information.
Moreover, the high-level attributes (\eg, pose, structure, and layout) and low-level attributes (\eg, color, texture, and style) are naturally disentangled. 
% Moreover, the high-level attributes (\eg, pose and structure) and low-level attributes (\eg, color and style) are naturally disentangled. 
%This facilitates applications such as style mixing and semantic interpolation with different paths.

\subsection{Disentangled Attribute Manipulation with Truncated Features}\label{subsec:disentangled}

A critical issue for image editing is the entanglement of features in the latent space.
For example, in face editing, ``old'' is often entangled with ``wearing glasses'', and ``arched eyebrows'' is often entangled with ``female''.
In this subsection, we investigate whether the feature entanglement is related with the normalized classifier weights $\hat{n}$, and propose an approach to disentangle attributes by adjusting $\hat{n}$.

As shown by the empirical Cumulative Distribution Function of the values of the normalized classifier weights $\hat{n}$ in Fig.~\ref{directionbarmap}, most values of $\hat{n}$ are relatively low, and only a few values are high.
%We also visualized normalized classifier direction $\hat{n}$ in the form of histogram, as shown in Fig.\ref{directionbarmap}.
%We can observe that most of the normalized classifier directions are relatively low, only few are notable.
%Based on these observations, we speculate that some notable directions can represent the main direction of this attribute.
We hypothesize that the high-value elements indicate the dominant direction of an attribute classifier, and other low-value elements are noisy and may lead to attribute entanglement.
We find that a truncated $n$ actually leads to better disentangled attribute manipulation.
In particular, we denote the set of the top-k largest values of $\hat{n}$ as $\text{top-k}(\hat{n})$, and truncate the values beyond the top-k largest ones.
\begin{equation}
    n^\prime_i=\left\{\begin{array}{l}
         n_i, \text{ if } \hat{n}_i\in  \text{top-k}(\hat{n})  \\
         0, \text{   else} 
    \end{array}
    \right.
\end{equation}

Our experiments in Fig.~\ref{topkmanipulate} validate that the truncated classifier direction $n^\prime$ facilitates disentangled image manipulation.
%And we rank the normalized classifier direction $\hat{n}$ in descending order to obtain notable directions.
%We assign the top $k$ ($0 \le k\le L \times 512$) normalized classifier directions to 1 and the rest to 0 to obtain a binary mask vector $m_k$ of dimension $512 \times L$.

%After that, we get the new normalized classifier direction $n_k$ as follows:
%\begin{align}
%    n_k = n \odot m_k
%\end{align}
%To manipulate the attribute of a synthesized image, we can edit the original latent code $z$ with $z_{edit} = z+\alpha n_k$.
%And we can change the value of $k$ ($0 \le k\le L \times 512$) to control the degree of disentanglement.
%As shown in Fig.\ref{topkmanipulate}, as $k$ decreases, the main manipulated attribute is slowly disentangled with other entangled attributes.
%Finally, different attributes can be completely disentangled when $k = 24$.
\label{sec:method}





==> section/05_experiment_.tex <==
\section{Experiments}
\subsection{Experimental settings}



% We conduct the experiments on the face datasets FFHQ~\cite{Stylegan} and CelebA-HQ~\cite{ProGAN}  for the face reconstruction.
Following Diffusion Autoencoders~\cite{DAE}, we train the hierarchical diffusion autoencoders on FFHQ~\cite{Stylegan} dataset and train the attribute classifiers on CelebA-HQ~\cite{ProGAN} dataset.
%The models are tested on CelebA-HQ dataset.

%as the test set for the face reconstruction experiment, as shown in Tab.~\ref{imgrectab}.

\input{figs/ablationplot}


%For the cat reconstruction, we adopt LSUN Cat~\cite{Lsun} and follow the official data splitting strategy.
The ablation study in Sec.\ref{sec:abl} is trained on $128 \times 128$ images and other results are derived from models trained on $256 \times 256$ images.
More implementation details can be found in Appendix.
%The Diffusion Autoencoders(DAE)~\cite{DAE} of different latent spaces are trained on 130M images of size $128 \times 128$ and use time steps $T=100$ for decoding.
%We also train our HDAE on 130M images of size $256 \times 256$ and use the original DAE which was trained on 200M images of size $256 \times 256$ to compare their image manipulation results.

\subsection{Ablation Study}\label{sec:abl}
We conduct ablation studies to test the effectiveness of the five design choices of diffusion autoencoders and hierarchical diffusion autoencoders demonstrated in Fig.\ref{overview}.
% We use 65k images from FFHQ dataset as the training set, and use the other 5k images from FFHQ dataset as the test set.
We use 65k images from the FFHQ dataset as the training set, and use the left 5k images as the test set.
We report the image reconstruction quality on the test set, evaluated by pixel-wise MSE and the perceptual quality, in Fig.\ref{ablationplot}.
%We carry out ablations on FFHQ~\cite{Stylegan} dataset using image reconstruction quality, as shown in Fig.\ref{ablationplot}.
%Pixel-wise MSE and perceptual LPIPS~\cite{LPIPS} are adopted as metrics to evaluate the image reconstruction quality.
%We use the former 65k FFHQ images of size $128 \times 128$ as the training set and 5k images of size $128 \times 128$ as the test set.
%We analyze the ablation experiments from the following four perspectives.
We draw the following conclusions based on the ablation study results:

\noindent\textit{The hierarchical network structures perform much significantly better than non-hierarchical ones.}
As illustrated in Fig.\ref{ablationplot}, all  the three variants of hierarchical diffusion autoencoders, HDAE(E), HDAE(U), and HDAE(U+), perform significantly better and converge much faster than DAE and DAE(U). The image reconstruction performances of HDAE(E) and HDAE(U) at 340K steps are better than the performances of DAE and DAE(U) at 1,020K steps.

\noindent\textit{The U-Net structure for the semantic encoder has a negative effect on DAE, but benefits HDAE.} As demonstrated in Fig.\ref{ablationplot}, DAE(U) performs worse than DAE, but HDAE(U) performs better than HDAE(E).

\noindent\textit{We select HDAE(U) as our best model architecture for further experiments}, as HDAE(U+) only performs marginally better than HDAE(U) with a cost of twice the latent space dimension.

% \paragraph{E space vs. ED space.}
%\noindent\textbf{DAE vs. DAE(U).}
% E space is the latent space used by the original Diffusion Autoencoders~\cite{DAE}. 
%Unlike DAE, DAE(U) uses a u-net~\cite{unet} like architecture semantic encoder. 
%As shown in Fig. \ref{ablationplot}, replacing the original encoder with u-net like architecture increases about $0.001$ on MSE metric. 
%And they are almost the same on LPIPS~\cite{LPIPS} metric. 
%It demonstrates that u-net like architecture semantic encoder cannot directly improve the performance of Diffusion Autoencoders.

\input{figs/Reconstruct}

% \paragraph{E space vs. E+ space.}

%\noindent\textbf{DAE vs. HDAE.}
%Instead of using one single semantic vector (DAE), HDAE uses hierarchical semantic vectors from feature maps at different scales. 
%As shown in Fig. \ref{ablationplot}, HDAE outperforms DAE at one third of the baseline DAE training time (40M steps).
%And HDAE decays about $0.003$ on MSE metric and $0.025$ on LPIPS~\cite{LPIPS} metric over DAE at 120M steps.
%It demonstrates that Hierarchical Diffusion Autoencoders is an efficient learner.

% \paragraph{E+ space vs. ED+ space.}
%\noindent\textbf{HDAE vs. HDAE(U).}
%Unlike HDAE, HDAE(U) not only uses hierarchical semantic vectors, but also uses an u-net~\cite{unet} like architecture semantic encoder instead of original encoder.
%As shown in Fig. \ref{ablationplot}, replacing the original encoder with u-net like architecture with hierarchical semantic vectors decays about $0.001$ on MSE metric and $0.005$ on LPIPS~\cite{LPIPS} metric. 
%It demonstrates that u-net like architecture semantic encoder can improve performance with Hierarchical Diffusion Autoencoders.

% \paragraph{ED+ space vs. ED++ space.}
%\noindent\textbf{HDAE(U) vs. HDAE(U+).}
%As shown in Fig. \ref{overview}, HDAE(U+) uses the feature maps from encoder and decoder in the semantic encoder, while HDAE(U) only uses the feature maps from decoder in the semantic encoder.
%Fig. \ref{ablationplot} shows that they are almost the same on LPIPS~\cite{LPIPS} and MSE.
%It demonstrates that only using the feature maps from decoder is enough to express the information contained in the input data and the feature maps from decoder are better than the feature maps from encoder.


% Furthermore, we conduct user studies to evaluate the performance of HDAE(U) and DAE in Tab. \ref{userstudytab}.
% % We collect 450 votes from 15 participants for the image reconstruction experiment and 1050 votes from 15 participants for the image manipulation experiment.
% We collect 450 and 1,050 votes from 15 participants for the image reconstruction experiment and the image manipulation experiment.
% The reported value indicates the preference rate of HDAE(U) against DAE.


\subsection{Image Reconstruction}
\input{tables/imgrectab}
\input{tables/userstudytab}
\noindent\textbf{Setup.}
We evaluate the reconstruction quality of following eight models: (1) pretrained StyleGAN2~\cite{Stylegan2} with \begin{math}\mathcal{W}\end{math} space, (2) pretrained StyleGAN2 with \begin{math}\mathcal{W+}\end{math} space, (3) VQ-GAN~\cite{VQGAN}, (4) HFGI~\cite{HFGI}, (5) VQ-VAE2~\cite{VQVAE2}, (6) DDIM~\cite{DDIM}, (7) DAE~\cite{DAE}, (8) our HDAE(U). Among those methods, (1)-(4) are GAN inversion approaches, (5) is a VAE-based approach, and (6)-(8) are diffusion-based methods.
All these models are trained on FFHQ~\cite{Stylegan} dataset and tested on 30k images from CelebA-HQ~\cite{ProGAN} dataset.
To validate the potential of our model beyond the face domain, we also demonstrate image reconstruction results on cat datasets by training the models on LSUN~\cite{Lsun} Cat dataset and testing on the AFHQ Cat~\cite{Starganv2} dataset for image reconstruction.
%We also train DAE and HDAE(U) on LSUN Cat~\cite{Lsun} and test them on AFHQ Cat~\cite{Starganv2} for the cat reconsturcion.
DDIM, DAE, and HDAE(U) are trained on images of size 128 × 128 and we use T=100 for inference. 
For the other models, we utilize the public available pretrained models and downsample the reconstructed images to $128 \times 128$ for comparison.
Structural Similarity SSIM, Pixel-wise MSE and perceptual quality metric LPIPS~\cite{LPIPS} are adopted to evaluate the image reconstruction quality.
%\xihui{discuss xT.}
To illustrate what information is encoded by the stochastic encoder, we show the images reconstructed from DAE and HDAE(U) with their corresponding $x_T$ as well as random $x_T$ for comparison.





\noindent\textbf{Quantitative results.}
The results Tab.\ref{imgrectab} demonstrate that: (1) our HDAE(U) achieves near-perfect image reconstruction performance, outperforming previous GAN inversion methods, VAE-based approaches, and diffusion-based approaches.
(2) Comparing image reconstruction results with the $x_T$ encoded by a stochastic encoder and random $x_T$, we draw the conclusion that some detail-related information is encoded by the stochastic encoder.
(3) The image reconstruction performance degrades more for DAE than HDAE(U) when replacing $x_T$ encoded by the stochastic encoder with a random $x_T$, indicating that the stochastic encoder of DAE encodes more information than HDAE(U).

%As shown in Tab.\ref{imgrectab}, HDAE(U) without stochastic code $x_T$ is well in excess of DAE without stochastic code $x_T$.
%It demonstrates that our Hierarchical Diffusion Autoencoders can capture more semantic information than original Diffusion Autoencoders to make semantic vectors suitable to express the information contained in the input data.
%And HDAE(U) achieves state-of-the-art performance with stochastic code $x_T$.



\input{figs/pro_interpolation}
\input{figs/interpolation}

\noindent\textbf{Qualitative results.}
We observe similar phenomenons from the qualitative results in Fig.\ref{Reconstruct}. Previous GAN inversion approaches PSP~\cite{PSP} and HFGI~\cite{HFGI} cannot preserve the background and details of the original image, while DAE and HDAE(U) produce reconstructed images nearly identical to the input images.
Comparing DAE with random $x_T$ with HDAE(U) with random $x_T$, we find that DAE(U) with random $x_T$ achieves preserves the background and details better. This observation indicates that the semantic encoder of HDAE(U) encodes more comprehensive features, allowing more fine-grained and controllable representations.


\noindent\textbf{Human perceptual evaluation.}
We conduct a human perceptual evaluation, where users are asked to vote for the image reconstruction quality of HDAE(U) with random $x_T$ and DAE with random $x_T$ in Tab.\ref{userstudytab}.
%\xihui{With $x_T$ or without $x_T$?}
We collect 450 votes from 15 participants, and the results are shown in Tab.\ref{userstudytab}.
Users clearly prefer the image reconstruction results by our HDAE(U) over DAE.
%indicates the preference rate of HDAE(U) against DAE.

%We show the visual results of face and cat inversion in Fig. \ref{Reconstruct}.
%Even though HFGI can restore the foreground of the given images, it struggles to reconstruct spatial details and the images reconstructed by HFGI are blurred.
%Thanks to Diffusion Autoencoders, DAE and HDAE(U) with stochastic code $x_T$ (2nd and 3rd row) provide higher quality images than HFGI (6th row).
%Although both HDAE(U) and DAE with stochastic code $x_T$ can provide high quality images, DAE without stochastic code struggles to reconstruct the input images.
%It demonstrates that a non-hierarchical semantic vector is not enough to express the information contained in the input data.
%Compared with DAE, HDAE(U) without stochastic code $x_T$ (5th row) preserves more details in backgrounds, appearance, expressions and identity information without stochastic code $x_T$, as shown in Fig. \ref{Reconstruct}.



\subsection{Interpreting the Hierarchical Latent Space}
Our hierarchical latent space naturally disentangles abstract, high-level attributes from low-level attributes.
We verify this property and visualize the coarse-to-fine features encoded in the hierarchical latent space by style mixing and controllable image interpolation experiments.

\noindent\textbf{Style mixing.}
To interpret the correspondences between the hierarchical latent space and the attributes at different abstract levels, we mix the  high-level latent codes $z_s^5,z_s^6$ from source image A(B) and the low-level latent codes $z_s^1, z_s^2, z_s^3, z_s^4$ from image B(A), and use the mixed latent codes to generate a new image.
Fig.~\ref{interpolation} shows a clear hierarchy of the latent space. $z_s^1, z_s^2, z_s^3, z_s^4$ control the spatial details such as background, color, and lighting, and  $z_s^5,z_s^6$ control the high-level semantic attributes related to image structure such as pose, gender, face shape, and eyeglasses.
%Using the semantic encoder of HDAE(U) trained on FFHQ~\cite{Stylegan} of image size $256 \times 256$, we can get the hierarchical semantic vectors $z_s = \left \{ z_{d}^{l} \right \}^L_{l=1} $.
%As shown in Fig. \ref{interpolation}, (a) presents examples of images synthesized by mixing two latent codes at a specified scale. 
%We can see that semantic vector $z^l_d$ at different scales controls meaningful high-level attributes of the image.
%The semantic vectors corresponding to coarse spatial resolutions ($8^2 \sim 16^2$) encode high-level semantic information such as pose, gender, face shape, and eyeglasses. 
%The semantic vectors corresponding to high spatial resolutions ($32^2 \sim 256^2$) encode low-level semantic information such as color scheme, smaller-scale facial features and microstructure.

\noindent\textbf{Controllable image interpolation.}
Image interpolation based on semantic codes is a common way to visualize and verify the properties of the latent space.
With our hierarchical latent space, we can control different paths of image interpolation, as shown in Fig. \ref{pro_interpolation}.
Given the leftmost and rightmost real images in red boxes,
in the first row, we interpolate from left to right by changing low-level features first and then high-level features.
In the second row, the interpolation is conducted in a reverse way, from high-level features to low-level features.
In the third row, we illustrate the continuous changes between the two images in the second row.
The controllable interpolation results indicate that 
$z_s^1,z_s^2,z_s^3$ mainly control the lighting and color, $z_s^4$ controls the background, $z_s^5$ mainly controls the gender and $z_s^6$ mainly controls the pose.
%, (b) and (c) present image blending results by mixing different latent codes from scale $8*8$ to a specified scale.
%We can see that it blends high-level semantic information(pose, gender, face shape, and eyeglasses) of two images in coarse resolution ($8^2 \sim 16^2$) and it blends low-level semantic information(color scheme, smaller scale facial features and microstructure) of two images at high spatial resolutions ($32^2 \sim 256^2$).

% \noindent\textbf{Multi-scale information are gradually disentangled into hierarchical representations.}



\input{figs/facemanipulate}

\subsection{Image Manipulation}
% \paragraph{Image manipulation.}
\noindent\textbf{Detail-preserving image manipulation.}
With the linear attribute classifiers for the latent codes, we can conduct image manipulation on real images by manipulating the semantic latent codes of real images with the classifier direction.
Fig.\ref{facemanipulate} shows the visual results of image manipulation on real images using four models: (1) GAN inversion approach HFGI~\cite{HFGI}, (2) StyleClip~\cite{Styleclip}, (3) our baseline DAE~\cite{DAE}, and (4) our proposed model HDAE(U).
%We first train the DAE and HDAE(U) on FFHQ~\cite{Stylegan} of image size $256 
%\times 256$. 
%After that, we fix the DAE and HDAE(U) and train the classifier on CelebA-HQ~\cite{ProGAN} of image size $256 \times 256$. 
%For the other two models, we use publicly available pre-trained models.
The DAE and HDAE(U) are trained on the FFHQ dataset, and the linear attribute classifiers are trained on the CelebA-HQ dataset.
As demonstrated in Fig.\ref{facemanipulate},
our HDAE(U) preserves the details (\eg, background, face identity, and the forehead pendant) of the input image better than other approaches.
%Compared with HFGI and StyleClip, HDAE(U) does not manipulate the whole image, but only part of the image, as shown in Fig. \ref{facemanipulate}.
%Compared with DAE, HDAE(U) is better in details.
%It demonstrates that HDAE(U) obtains more disentangled representation and has higher fidelity than other models.
% It demonstrates that hierarchical semantic representation is more disentangled than other representation.

Furthermore, we conduct a user perceptual evaluation on the image manipulation results of HDAE(U) and DAE.
% We collect 450 votes from 15 participants for the image reconstruction experiment and 1050 votes from 15 participants for the image manipulation experiment.
We collect 1,050 votes from 15 participants, and the results in Tab.\ref{userstudytab} indicate that HDAE(U) performs better than DAE on image manipulation.


% \paragraph{Controllable disentangled image manipulation.}
\noindent\textbf{Disentangled image manipulation with truncated features.}
%Different attributes are often entangled when manipulating images, such as the attribute of "old" is often entangled with the attribute of "wearing glasses" and the attribute of "Arched Eyebrows" is often entangled with the attribute of "make up", as shown in Fig. \ref{topkmanipulate}.
%We propose a simple method to control the degree of disentanglement with hierarchical Diffusion Autoencoders.
As introduced in Sec.\ref{subsec:disentangled}, we leverage the truncated features for disentangled image manipulation.
We compare the qualitative results of image manipulation with truncated features ($k=24$ and $k=96$) and all feature channels ($k=3072$).
As shown in Fig.\ref{topkmanipulate}, the truncated features with $k=24$ effectively disentangle the attributes for manipulation. The attributes become more entangled as $k$ increases. For the na\"ive manipulation without truncated features, ``old'' is entangled with ``eyeglasses'', ``arched eyebrows'' is entangled with ``female'', and ``female'' is entangled with ``makeup''.
%We can see that as $k$ decreases, the main manipulated attribute is slowly disentangled with other entangled attributes.
%Finally, different attributes can be completely disentangled when $k = 24$.
%And we can change the value of $k$ ($0 \le k\le L \times 512$) to control the degree of disentanglement.


% \input{figs/gen_DAE(ED+)}

%\subsection{Image interpolation and blending}





\subsection{Other Applications}
%We show further applications of HAE on semantic image synthesis and unconditional image synthesis in the Appendix.
\noindent\textbf{Multi-modal semantic image synthesis.}
We train an extra layout encoder to map the semantic label map into the latent space of our HDAE.
Our HDAE can synthesize images based on the high-level features from the semantic label map and the low-level features from a real image. In this way, we can control the layout of the generated images with the label map, and control the image style and details with the image, as shown in Fig.~\ref{s2i}.
%Our HDAE can conduct multi-modal semantic image synthesis where the layout information is from the semantic segmentation map and the details from a source image.
%In other words, we can use the an style image to control the semantic image synthesis results.
%We can use HDAE(U) to transform semantic layouts into realistic images.
%To fully leverage the semantic information, the semantic label map is injected into the semantic encoder to obtain semantic vectors $z_s = \left \{ z_{d}^{l} \right \}^L_{l=1} $.
%And we can sample a noisy image and feed the noisy image into the diffusion u-net with semantic vectors $z_s$ to generate a realistic image.
%We train the HDAE(U) on CelebAMask-HQ~\cite{maskgan} dataset of image size $256 \times 256$.
%As shown in Fig. \ref{s2i}, HDAE(U) can produce a superior performance on fidelity and learned correspondence without any special design for this task.

\input{figs/s2i}

\noindent\textbf{Unconditional image synthesis.}
By training a DDIM model to predict the hierarchical latent codes, our model can be leveraged for unconditional image synthesis. Examples are shown in the Appendix.

\label{sec:experiments}



==> tables/_imgrectab.tex <==
% \begin{table}[t]
% \centering
% % \resizebox{\columnwidth}{!}{%

% \begin{tabular}{lc}
% \toprule
% Method & Accuracy \\
% \midrule
% Ours & 0.502 \\
% \bottomrule
% \end{tabular}

% % }
% \caption{
% Caption goes here
% }
% \vspace{-0.05in}
% \label{tab:template}
% \end{table}


% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\resizebox{1\linewidth}{!}{
    \begin{tabular}{lc|c|ccc}
    % \hline
    \toprule[1.2pt]
    \textbf{Model} & \textbf{Setting}  & \textbf{Latent dim} & \textbf{SSIM$\uparrow$}                & \textbf{LPIPS$\downarrow$}               & \textbf{MSE$\downarrow$}                   \\ \midrule[1.2pt]
    StyleGAN2\begin{math}(\mathcal{W})\end{math}~\cite{Stylegan2} &  -   & 512                 & 0.677                        & 0.168                        & 0.016                          \\
    StyleGAN2\begin{math}(\mathcal{W+})\end{math}~\cite{Stylegan2} &  -  & 7168                & 0.827                        & 0.114                        & 0.006                          \\
    VQ-GAN~\cite{VQGAN}&      -      & 65536               & 0.782                        & 0.109                        & 3.61e-3                        \\
    VQ-VAE2~\cite{VQVAE2}&     -      & 327680              & 0.947                        & 0.012                        & 4.87e-4                        \\
    HFGI~\cite{HFGI} & - & 7168 & 0.877 & 0.127 & 0.0617 \\
    DDIM~\cite{DDIM} & T=100, $128^2$             & 49512               & 0.917                        & 0.063                        & 0.002                          \\ \midrule[1.2pt]
    DAE~\cite{DAE} & T=100, $128^2$, random $x_T$   & 512                 & 0.677                        & 0.073                        & 0.007                          \\
    \textbf{HDAE(U) (ours)} & T=100, $128^2$, random $x_T$ & 2560                &  0.793 &  0.038 &  2.96e-3 \\ \midrule[1.2pt]
    DAE~\cite{DAE} & T=100, $128^2$, encoded $x_T$   & 49664               & 0.991                        & 0.011                        & 6.07e-5                        \\
    \textbf{HDAE(U) (ours)} & T=100, $128^2$, encoded $x_T$ & 52072               & \textbf{0.993}               & \textbf{0.009}               & \textbf{5.01e-5}               \\ 
    % \hline
    \bottomrule[1.2pt]
    \end{tabular}
}
\caption{
    \textbf{Image reconstruction evaluation of models trained on FFHQ~\cite{Stylegan} and tested on CelebA-HQ~\cite{ProGAN}.}
    % HDAE(U) outperforms DAE with random stochastic code $x_T$, indicating that the semantic latent space of HDAE(U) encodes richer details than DAE.
    HDAE(U) outperforms DAE with random stochastic code $x_T$, indicating that HDAE(U) encodes richer details than DAE.
    HDAE(U) with encoded $x_T$ achieves state-of-the-art, near-perfect reconstruction results.
}
\vspace{-0.3cm}
\label{imgrectab}
\end{table}

==> tables_rebuttal/tab_dae_and_hdae_linear_probe.tex <==
% \begin{table}[t]
% \resizebox{1\linewidth}{!}{
% \begin{tabular}{l|cccccccc|c}
% \hline
%        & \multicolumn{8}{c|}{Some attributes}                                                          &               \\
% Method & Big\_Nose & Big\_Lips & Young  & Smile  & Eveglass & Blackhair & Arched\_Eyebrows & Brownhair & Macro average \\ \hline
% DAE    & 0.8293    & 0.692     & 0.8772 & 0.9686 & 0.965    & 0.8866    & 0.8243           & 0.7872    & 0.8785        \\
% HDAE   & 0.8443    & 0.7205    & 0.8831 & 0.9711 & 0.9691   & 0.8887    & 0.8392           & 0.8234    & 0.8823        \\ \hline
% \end{tabular}
% }
% \caption{}
% \label{dae_and_hdae_linear_probe}
% \end{table}


\begin{table}[t]
\renewcommand\arraystretch{1.4}
\resizebox{1\linewidth}{!}{
\begin{tabular}{l|cccc}
\hline
Method       & DAE   & HDAE  & HDAE low-level code & HDAE high-level code \\ \hline
Accuracy(\%) & 61.85 & 66.34 & 50.05               & 65.30                \\ \hline
\end{tabular}
}
\vskip -0.05in
\caption{}
\label{dae_and_hdae_linear_probe}
\vskip -0.1in
\end{table}

% \begin{table}[]
% \begin{tabular}{l|llll}
% \hline
% Method       & DAE   & HDAE  & HDAE low-level code & HDAE high-level code \\ \hline
% Accuracy(\%) & 61.85 & 66.34 & 50.05               & 65.30                \\ \hline
% \end{tabular}
% \caption{}
% \label{tab:my-table}
% \end{table}

==> tables_rebuttal/tab_low_high_linear_probe.tex <==
\begin{table}[]
% \vskip -0.1in
\renewcommand\arraystretch{1.4}
\resizebox{1\linewidth}{!}{
\begin{tabular}{l|cccc|cccc|c}
\hline
\multirow{2}{*}{Method} & \multicolumn{4}{c|}{Attributes related to high-level} & \multicolumn{4}{c|}{Attributes related to low-level}  & \multicolumn{1}{c}{Macro average} \\
                        & Smile      & Eveglass    & Oval\_Face    & Young     & Blackhair & PaleSkin & Brownhair & 5\_o\_Clock\_Shadow &  on all attributes                              \\ \hline
HDAE Low-level code                     & 0.8874     & 0.894       & 0.6397        & 0.8537    & \uline{0.8867}    & \uline{0.9107}   & \uline{0.8196}    & \uline{0.8938}              & 0.8418                         \\
HDAE High-level code                    & \uline{0.9705}     & \uline{0.9552}      & \textbf{0.668}         & \uline{0.8659}    & 0.789     & 0.7809   & 0.673     & 0.8535              & 0.8452                         \\
HDAE Whole code                     & \textbf{0.9711}     & \textbf{0.9691}      & \uline{0.665}         & \textbf{0.8831}    & \textbf{0.8887}    & \textbf{0.928}    & \textbf{0.8234}     & \textbf{0.9067}              & \textbf{0.8823}                         \\ \hline
% DAE                     & 0.9686     & 0.965      & 0.6732         & 0.8772    & 0.8866    & 0.9399    & 0.7872     & 0.8985              & 0.8785 \\
DAE(2560)& 0.9651     & 0.9663      & 0.6456         & 0.8771    & 0.8797    & 0.9202    & 0.7852     & 0.8959              & 0.8673\\ 
\hline



\end{tabular}
}
\vskip -0.05in
\caption{\textgreenrv{ }\textbf{Q3} Linear probing on 40 attributes of CelebA-HQ.}
\label{tab_low_high_linear_probe}
\vskip -0.15in
\end{table}













% \begin{table}[t]
% \renewcommand\arraystretch{1.4}
% \resizebox{1\linewidth}{!}{
% \begin{tabular}{l|cccc}
% \hline
% Method       & DAE   & HDAE  & HDAE low-level code & HDAE high-level code \\ \hline
% Accuracy(\%) & 61.85 & 66.34 & 50.05               & 65.30                \\ \hline
% \end{tabular}
% }
% \vskip -0.05in
% \caption{}
% \label{dae_and_hdae_linear_probe}
% \vskip -0.1in
% \end{table}

% Method       & DAE & DAE(2560)   & HDAE \\ \hline
% Accuracy(\%) & 61.85 & 66.34 & 50.05               & 65.30                \\ \hline
